DreamCatalyst: Fast and High-Quality 3D Editing via Controlling Editability and Identity Preservation

Score distillation sampling (SDS) has emerged as an effective framework in text-driven 3D editing tasks, leveraging diffusion models for 3D-consistent editing. However, existing SDS-based 3D editing methods suffer from long training times and produce low-quality results. We identify that the root cause of this performance degradation is \textit{their conflict with the sampling dynamics of diffusion models}. Addressing this conflict allows us to treat SDS as a diffusion reverse process for 3D editing via sampling from data space. In contrast, existing methods naively distill the score function using diffusion models. From these insights, we propose DreamCatalyst, a novel framework that considers these sampling dynamics in the SDS framework. Specifically, we devise the optimization process of our DreamCatalyst to approximate the diffusion reverse process in editing tasks, thereby aligning with diffusion sampling dynamics. As a result, DreamCatalyst successfully reduces training time and improves editing quality. Our method offers two modes: (1) a fast mode that edits Neural Radiance Fields (NeRF) scenes approximately 23 times faster than current state-of-the-art NeRF editing methods, and (2) a high-quality mode that produces superior results about 8 times faster than these methods. Notably, our high-quality mode outperforms current state-of-the-art NeRF editing methods in terms of both speed and quality. DreamCatalyst also surpasses the state-of-the-art 3D Gaussian Splatting (3DGS) editing methods, establishing itself as an effective and model-agnostic 3D editing solution. See more extensive results on our project page: https://dream-catalyst.github.io.

==> assets/comparison_plot.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray196}{RGB}{196,196,196}
\definecolor{lightgray204}{RGB}{204,204,204}
\pgfplotsset{minor grid style={dotted,lightgray204}}

\begin{axis}[
width=\textwidth,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray196},
xlabel={Timesteps ($t$)},
xmajorgrids,
xmin=-50, xmax=1050,
xtick={0, 200, ...,1000},
xticklabels={0,200,400,600,800,1000},
xminorgrids,
minor xtick={0,100,...,1000},
% xtick style={color=black},
% y grid style={darkgray196},
ylabel={Magnitudes},
ymajorgrids,
ymin=-0.15, ymax=1.4,
yminorgrids,
minor ytick={0,0.25,...,1.25},
ytick style={color=black},
tick label style={font=\tiny},
label style={font=\small}
]
\addplot[color=blue, thick] table[x=t, y=phi, col sep=comma] {assets/new_coefficients_timestep.csv};
\addlegendentry{$\Phi^{*}$}
\addplot[color=red, thick] table[x=t, y=psi, col sep=comma] {assets/new_coefficients_timestep.csv};
\addlegendentry{$\Psi^{*}$}
\end{axis}

\end{tikzpicture}


==> assets/evaluation_prompt_oneline_small.tex <==
\begin{table} [t!]
  \footnotesize
  \newcommand{\xpm}[1]{{\tiny$\pm#1$}}
  \newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
  \centering
\setlength{\tabcolsep}{2.7pt}
\begin{small}
\scalebox{0.65} {

% \begin{tabular}{@{}c P{3.0cm} P{4.4cm} P{4.6cm}@{}}
\begin{tabular}{@{}c c c c@{}}
  \toprule
  Scene  & Source Prompt  & Target Prompt (Description)  & Target Prompt (Instruction)  \\
    \midrule
    Face &  ``a photo of a face'' & ``a photo of the Tolkien Elf'' & ``Turn him into the Tolkien Elf'' \\
    Face &  ``a photo of a face'' & ``a photo of the Emma Watson'' & ``Turn him into Emma Watson'' \\
    Face &  ``a photo of a face'' & ``a photo of Elon Musk'' & ``Turn him into Elon Musk'' \\
    Face &  ``a photo of a face'' & ``a photo of an Einstein'' & ``Turn him into an Einstein'' \\
    Face &  ``a photo of a face'' & ``a photo of a face with mustache'' & ``Give him a mustache'' \\
    Face &  ``a photo of a face'' & ``a photo of Leonardo Dicaprio'' & ``Turn him into Leonardo Dicaprio'' \\
    Face &  ``a photo of a face'' & ``a photo of a skull'' & ``Turn his face into a skull'' \\
    Bear &  ``a photo of a bear statue'' & ``a photo of a grizzly bear'' & ``Turn the bear statue into a grizzly bear'' \\
    Bear &  ``a photo of a bear statue'' & ``a photo of a panda'' & ``Turn the bear statue into a panda'' \\
    Bear &  ``a photo of a bear statue'' & ``a photo of an asiatic black bear'' & ``Turn the bear statue into an asiatic black bear'' \\
    Bear &  ``a photo of a bear statue'' & ``a photo of a polar bear'' & ``Turn the bear statue into a polar bear'' \\
    Bear &  ``a photo of a bear statue'' & ``a photo of a Bengal tiger'' & ``Turn the bear statue into a Bengal tiger'' \\
    Bear &  ``a photo of a bear statue'' & ``a photo of a skull bear'' & ``Turn the bear statue into a skull bear'' \\
    Person &  ``a photo of a person'' & ``a photo of a Super Mario'' & ``Turn him into a Super Mario'' \\
    Person &  ``a photo of a person'' & ``a photo of a clown'' & ``Turn him into a clown'' \\
    Person &  ``a photo of a person'' & ``a photo of a person reading a book'' & ``Make him reading a book'' \\
    Person &  ``a photo of a person'' & ``a photo of a person wearing a sunglass'' & ``Wear him a sunglass'' \\
    Person &  ``a photo of a person'' & ``a photo of a Storm Trooper'' & ``Turn him into a Storm Trooper'' \\
    Person &  ``a photo of a person'' & ``a photo of Elon Musk'' & ``Turn him into Elon Musk'' \\
    Person &  ``a photo of a person'' & ``a photo of an Iron Man'' & ``Turn him into an Iron Man'' \\
    Person &  ``a photo of a person'' & ``a photo of a Jack Sparrow'' & ``Turn him into a Jack Sparrow'' \\
    Person &  ``a photo of a person'' & ``a photo of a bronze statue'' & ``Make him into a bronze statue'' \\
    Plant &  ``a photo of a plant'' & ``a photo of a rose above the flowerpot with soil'' & ``Turn only the plant above the flowerpot into a rose and keep soil'' \\
    Plant &  ``a photo of a plant'' & ``a photo of a sunflower above the flowerpot with soil'' & ``Turn only the plant above the flowerpot into a sunflower and keep soil'' \\
    Plant &  ``a photo of a plant'' & ``a photo of a tulip above the flowerpot with soil'' & ``Turn only the plant above the flowerpot into a tulip and keep soil'' \\
    Bamboo &  ``a photo of a bamboo'' & ``a photo of an orange tree with oranges'' & ``Turn the tree into an orange tree with oranges'' \\
    Campsite &  ``a photo of a campsite'' & ``a photo of a campsite just snowed'' & ``Make it look like it just snowed'' \\
    Campsite &  ``a photo of a campsite'' & ``a photo of a campsite at sunset'' & ``Make it sunset'' \\
    Farm &  ``a photo of a farm'' & ``a photo of a farm in autumn'' & ``Make it autumn'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of a Batman'' & ``Turn him into a Batman'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of a Marvel's Spider-Man'' & ``Turn him into a Marvel's Spider-Man'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of a clown'' & ``Turn him into a clown'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of a Joker'' & ``Turn him into a Joker'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of a Hulk'' & ``Turn him into a Hulk'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of a Thanos'' & ``Turn him into a Thanos'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of Leonardo Dicaprio'' & ``Turn him into Leonardo Dicaprio'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of a Darth Vader'' & ``Turn him into a Darth Vader'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of a Storm Trooper'' & ``Turn him into a Storm Trooper'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of a Deadpool'' & ``Turn him into a Deadpool'' \\
    Yuseung &  ``a photo of a man'' & ``a photo of a baldman'' & ``Make him a bald'' \\
  \bottomrule
\end{tabular}
}
\end{small}

\vspace{0.5em}
\caption{\textbf{Detailed evaluation text prompts.} The description-style prompts are used for PDS, which employs the Stable Diffusion model~\citep{rombach2022high_stable_diffusion}, while the instruction-style prompts are applied to IN2N, GE, DGE, and our method, all of which utilize the InstructPix2Pix model~\citep{brooks2023instructpix2pix}.}
\label{table:evaluation_text_prompt}
\end{table}

